Parallelising Glauber dynamics

For distributions over discrete product spaces $\prod_{i=1}^n \Omega_i'$, Glauber dynamics is a Markov chain that at each step, resamples a random coordinate conditioned on the other coordinates. We show that $k$-Glauber dynamics, which resamples a random subset of $k$ coordinates, mixes $k$ times faster in $\chi^2$-divergence, and assuming approximate tensorization of entropy, mixes $k$ times faster in KL-divergence. We apply this to obtain parallel algorithms in two settings: (1) For the Ising model $\mu_{J,h}(x)\propto \exp(\frac1 2\left\langle x,Jx \right\rangle + \langle h,x\rangle)$ with $\|J\|<1-c$ (the regime where fast mixing is known), we show that we can implement each step of $\widetilde \Theta(n/\|J\|_F)$-Glauber dynamics efficiently with a parallel algorithm, resulting in a parallel algorithm with running time $\widetilde O(\|J\|_F) = \widetilde O(\sqrt n)$. (2) For the mixed $p$-spin model at high enough temperature, we show that with high probability we can implement each step of $\widetilde \Theta(\sqrt n)$-Glauber dynamics efficiently and obtain running time $\widetilde O(\sqrt n)$.

==> ack.tex <==
\section*{Acknowledgements}

Thanks to Leo Du for motivating the problem, to Frederic Koehler and Nicolas Loizou for helpful discussions, and to an anonymous reviewer for bringing the results of \cite{liu2022simple} to our attention.
%(FK for suggesting Theorem~\ref{t:atoe-ising}).

==> gd.tex <==
\section{Convergence of gradient descent}
\label{s:gd}

\begin{proof}[Proof of Lemma~\ref{l:gd}]
    Let $\ga=\fc{c}{L^2}$ denote the step size. Let $\De(x) = F(x-\ga F(x))-F(x)$. 
    Then $c$-strong monotonicity gives
    \begin{align*}
        \an{\De(x) , -\ga F(x)} &\ge c\ve{-\ga F(x)}^2\\
        \implies 
        \an{\De(x), F(x)}&\le -c\ga \ve{F(x)}^2. 
    \end{align*}
    By $L$-Lipschitzness, $\ve{\De(x)}\le \ga L\ve{F(x)}$. Hence
    \begin{align*}
        \ve{F(x-\ga F(x))}^2& = \an{F(x)+\De(x), F(x)+\De(x)}\\
        &\le \ve{F(x)}^2 - 2c\ga \ve{F(x)}^2 + \ve{\De(x)}^2\\
        &\le \pa{1-2c\ga + \ga^2 L^2} \ve{F(x)}^2\\
        &= \pa{1-\fc{c^2}{L^2}}\ve{F(x)}^2.
    \end{align*}
    This shows the per-iterate decrease, giving the desired linear convergence.
\end{proof}
